An exploratory study on how Internet of Things developing companies handle User Experience Requirements

[Context and motivation] Internet of Things (IoT) is becoming common throughout everyday lives. However, the interaction is often different from when using e.g. computers and other smart devices. Furthermore, an IoT device is often dependent on several other systems, heavily impacting the user experience (UX). Finally, the domain is changing rapidly and is driven by technological innovation. [Question/problem] In this qualitative study, we explore how companies elicit UX requirements in the context of IoT. A key part of contemporary IoT development is also data-driven approaches. Thus, these are also considered in the study. [Principal idea / Results] There is a knowledge gap around data-driven methodologies, there are examples of companies that collect large amount of data but do not always know how to utilize it. Furthermore, many of the companies struggle to handle the larger system context, where their products and the UX they control are only one part of the complete IoT ecosystem. [Contribution] We provide qualitative empirical data from IoT developing companies. Based on our findings, we identify challenges for the companies and areas for future work.

==> tab1.tex <==
% This is just to keep a copy of old table for sake of reference. 

\begin{table}[!hbt]
\centering
\caption{Participating companies. Category (Cat.): P = Product company, C = Consulting company. The size of the companies are displayed as number of employees, and the age in years.}\label{tab:total}.
\begin{tabular}{l l l l l l l}
\hline
\rule{0pt}{4ex}
\textbf{Id} & \textbf{Size} & \textbf{Age} & \textbf{Cat.} & \textbf{Industry} & \textbf{Interviewee(s)}\\
\hline
\hline
A & 600 & 30 & C & \pbox{20cm}{Specialised in embedded systems.\\Operating in industrial automation\\and product development\\} & \pbox{20cm}{Senior software\\developer}\\
B & 270 & 4 & C & \pbox{20cm}{Design and product development\\of IoT technology within\\e.g. interior, automotive, health care\\} & Head of Design\\
C & 8 & 2 & C & \pbox{20cm}{Specialised in IoT with focus on\\industrial IoT, e-health, energy} & \pbox{20cm}{C1: CEO, \\C2: Industrial Designer}\\\\
D & 10 & 4 & P & \pbox{20cm}{Start-up company with an edge-\\processing sensor used within retail \\and facility mgmt} & Sales Director\\
E & 45 & 30 & C & \pbox{20cm}{Product development within IoT\\and other areas\\} & \pbox{20cm}{E1: SW Developer, \\E2: R$\&$D Manager}\\
F & 4000 & 40 & C & \pbox{20cm}{Global IT management company.\\Provides IT solutions and services} & Lead of IoT\\\\
G & 10 & 2 & C & \pbox{20cm}{Design studio. Develops concepts,\\pitches, stories, and visions} & Lead Interaction Designer\\\\
H & 100 & 2 & P & \pbox{20cm}{International mobile communication\\company with a separate innovation\\department} & Senior UX Designer\\
I & 30 & 2 & P & Start-up automotive company & Software Developer\\
J & 70 & 2 & P & Development of smart B2C products & UX Director\\
K & 9 & 3 & P & \pbox{20cm}{Start-up company with a home\\security system} & CEO\\
\hline 
\end{tabular} 
\end{table}


==> tab2.tex <==
% This is just to keep a copy of original table for sake of reference. 

\begin{table}[!hbt]
\centering
\caption{UX activities during the development process, Category (Cat.): P = Product company, C = Consulting company}\label{tab:ux_activities}
\begin{tabular}{l l l l}
\textbf{Id} & \textbf{Cat.} & \textbf{\pbox{20cm}{Qualitative activities}} &  \textbf{\pbox{20cm}{Quantitative activities}} \\
\hline
A & C & - & \pbox{20cm}{-} \\

B & C & \pbox{20cm}{Prototyping \\ User tests \\} & \pbox{20cm}{User data \\}\\
 
C & C & \pbox{20cm}{Prototyping \\} & \pbox{20cm}{-\\}\\

D & P & \pbox{20cm}{Prototyping \\} & \pbox{20cm}{Unknown} \\

E & C & \pbox{20cm}{Occasional user tests} & \pbox{20cm}{-} \\

F & C & \pbox{20cm}{Depends on the customer\\ Mock-ups \\User feedback\\} & \pbox{20cm}{-\\} \\

G & C & \pbox{20cm}{User research\\ User tests\\ Scenarios\\ Story boards\\ Personas\\} & \pbox{20cm}{User data\\ A/B testing\\} \\

H & P  & \pbox{20cm}{Prototype/Simulation\\End user tests \\ Personas \\ Surveys \\ Interviews with end users\\} & \pbox{20cm}{Google Analytics\\A/B testing \\}  \\

I & P & \pbox{20cm}{Indirect user feedback\\Conceptual schetches\\} & - \\ \\

J & P & \pbox{20cm}{User research\\Feedback from beta testers \\ Personas \\ Focus Groups \\ Sketches \\} & \pbox{20cm}{Google Analytics \\ In-house A/B testing} \\

K & P & \pbox{20cm}{User research\\User feedback\\Prototyping} & Unknown \\

\hline

\end{tabular} 
\end{table}

